Best-Response Dynamics and Fictitious Play in Identical-Interest and Zero-Sum Stochastic Games

This paper combines ideas from Q-learning and fictitious play to define three reinforcement learning procedures which converge to the set of stationary mixed Nash equilibria in identical interest discounted stochastic games. First, we analyse three continuous-time systems that generalize the best-response dynamics defined by Leslie et al. for zero-sum discounted stochastic games. Under some assumptions depending on the system, the dynamics are shown to converge to the set of stationary equilibria in identical interest discounted stochastic games. Then, we introduce three analog discrete-time procedures in the spirit of Sayin et al. and demonstrate their convergence to the set of stationary equilibria using our results in continuous time together with stochastic approximation techniques. Some numerical experiments complement our theoretical findings.

==> include/abstract.tex <==

This paper combines ideas from $Q$-learning~\cite{watkinsTechnicalNoteQLearning1992} and fictitious play~\cite{brown1951iterative, robinsonIterativeMethodSolving1951, mondererFictitiousPlayProperty1996} to define three reinforcement learning procedures which converge to the set of stationary mixed Nash equilibria in identical interest discounted stochastic games. First, we analyse three continuous-time systems that generalize the best-response dynamics defined by~\citet{leslieBestresponseDynamicsZerosum2020} for zero-sum discounted stochastic games. Under some assumptions depending on the system, the dynamics are shown to converge to the set of stationary equilibria in identical interest discounted stochastic games. Then, we introduce three analog discrete-time procedures in the spirit of~\citet{sayinFictitiousPlayZerosum2020} and demonstrate their convergence to the set of stationary equilibria using our results in continuous time together with stochastic approximation techniques \cite{benaimStochasticApproximationsDifferential2005}. Some numerical experiments complement our theoretical findings.


==> include/simulations.tex <==
\hypertarget{sec:simulations}{%
\section{Extensions and Simulations}
\label{sec:simulations}}

\paragraph{Generalization of fictitious play}

The procedure we defined in the previous section is a special case of a more general procedure \iffalse parameterized by a function $\alpha$ that is, similarly to the best-response dynamics outlined in Section~\ref{sec:brd}, the update rate of the payoff estimate. The generalized estimate is\fi defined as follows:

\[\dui {n+1} s := \left(\sum\limits_{k=0}^{\countsn}\frac{1}{\alpha(k)}\right)^{-1}\sum\limits_{k=0}^n\frac{\indic {s_k} s}{\alpha(s^\sharp_k)}\stfis {u^i_k}{x_{k,s}}\]
where $\alpha$ is supposed non-decreasing. The former estimate corresponds to the case where $\alpha$ is the constant function equal to one.

This latest estimate would be the counterpart to the continuous system studied in the previous section. However, the link between the continuous and discrete systems is not straightforward. Therefore the convergence of the general version for identical interest games remains an open problem: the continuous system is non-autonomous and there is no general theory of stochastic approximations for such systems. An option could be to use two-timescale stochastic optimizations in the spirit of the work of \citet{borkarStochasticApproximationTwo1997} in a way similar to \citet{sayinFictitiousPlayZerosum2020}. However, there are regularities assumptions satisfied in zero-sum stochastic games that are not trivial to verify in our case and the continuous time systems would be different.

\RL{Il serait judicieux de rappeler que Leslie ne demontre pas la convergene du system discret mais seulement le system continue probablement pour la meme difficulte technique que toi}


We now describe the simulations that we have conducted in order to assess the two conjectures that we made namely the case $\delta \geq 1/|S|$ for \ref{eq:abrd} of Theorem~\ref{thm:contasync} and $\alpha(k) \neq 1$ for Theorem~\ref{thm:discrasync}. They were all run on a personal computer (Intel i5) in less than one hour.

\paragraph{Asynchronous continuous time system when $\delta \geq 1/|S|$}

We ran a simulation of differential inclusion~\ref{eq:abrd} using a simple Euler method. Our extensive simulations suggest that the system always converges for any randomly generated game. If our conjectures were disproved, then we believe that it would occur in very intricate cases such as degenerated stochastic games or with more players, actions and states. It is also possible that the system does not converge when rates $\ratest s t$ are correlated, which is especially difficult to simulate with a randomization. For the sake of readability, our figures only contain the $u_s$, but actions converge quickly towards a pure action profile. There may be several equilibria, so the system does not always converge to the same one.

The random games that we study have 2 actions, 2 states and 2 players.  We randomly chose an instance so as it is completely reproducible and plotted $u_1$, $u_2$, $\Delta_1$, $\Delta_2$ on Figure \ref{fig:cont} where $\Delta_s := f_{s, u}(x)-u_s$ is the error in the Bellman equation ($\Delta_s = 0$ would mean that $u_1$ and $u_2$ are solutions of the Bellman equation). Other instances can be tried in the notebook in the supplementary material. This is the instance chosen as example:
\begin{center}
    $P_1 = \left[\begin{matrix}
        0.09 & 0.05 \\ 0.95 & 0.79 
        \end{matrix}\right]$  $P_2 =\left[\begin{matrix}
        0.20 & 0.66 \\ 0.79 & 0.54 
        \end{matrix}\right]$  $r_1 = \left[\begin{matrix}
        0.65 & 0.37 \\ 0.00 & 0.73 
        \end{matrix}\right]$ $r_2 = \left[\begin{matrix}
        0.19 & 0.07 \\ 0.30 & 0.07 
        \end{matrix}\right]$ $\delta = 0.7$
    \end{center}
\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{alpha_1.png}
\includegraphics[width=0.45\textwidth]{alpha_t.png}
\caption{Simulation of the asynchronous best-response dynamics \ref{eq:abrd} for $\alpha(t) = 1$ (top) and $\alpha(t) = t+1$ (bottom)}\label{fig:cont}
\Description{Simulations show that all variables converge to a value, although at a different speed.}
\end{figure}

The notebook of the simulation in the supplementary material and plots in Appendix~\ref{app:plots} show that actions also converge. Vector $(u_1, u_2)$ converges towards $(0.50, 0.42)$ which is the payoff of the stationary strategy that actions $x^i_s$ converge to (see the notebook and Appendix~\ref{app:plots}). This stationary strategy is a stationary Nash equilibrium of the stochastic game: it is verified in the notebook by computing the discounted payoff of every pure strategy. Thus we conjecture that Theorem~\ref{thm:contasync} holds for $\delta \geq 1/|S|$. Furthermore, the continuous time system with $\alpha(t)=1$ converges, in the simulations, more rapidly than the one with $\alpha(t)=t+1$.

\paragraph{Fictitious play with two timescales} We ran our procedure \ref{eq:abrd} on the previous instance with $\alpha(k)=1$ and $\alpha(k)=k+1$. Compared to \ref{eq:abrd} with $\alpha(t)=1$, fictitious play with $\alpha(k)=1$ converges exponentially slower (which is predicted by the theory of stochastic approximations). Since fictitious play with $\alpha(k)=k+1$ converges exponentially slower compared to the version with $\alpha(k)=1$, this results in a double exponential slowdown. Figure~\ref{fig:discr} shows simulations of this system with a logarithmic scale on the time coordinate and different time scales on every graph. Similarly to the continuous time systems, vector $u$ converges to an equilibrium payoff which is $(0.50, 0.42)$ but other equilibria exist (see the notebook and Appendix~\ref{app:plots} for details).

\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{discr_alpha_1.png}
\includegraphics[width=0.45\textwidth]{discr_alpha_log.png}
\caption{A fictitious play process \ref{eq:afp} with $\alpha(k) = 1$ (top) and $\alpha(k) = k+1 $ (bottom)}
\label{fig:discr}
\Description{Simulations show that all variables converge to a value, although at a different speed.}
\end{figure}    
